Jiffy: A Lock-free Skip List with Batch Updates and Snapshots

In this paper we introduce Jiffy, the first lock-free, linearizable ordered key-value index that offers both (1) batch updates, which are put and remove operations that are executed atomically, and (2) consistent snapshots used by, e.g., range scan operations. Jiffy is built as a multiversioned lock-free skip list and relies on CPU's Time Stamp Counter register to generate version numbers at minimal cost. For faster skip list traversals and better utilization of the CPU caches, key-value entries are grouped into immutable objects called revisions. Moreover, by changing the size of revisions and thus modifying the synchronization granularity, our index can adapt to varying contentions levels (smaller revisions are more suited for write-heavy workloads whereas large revisions benefit read-dominated workloads, especially when they feature many range scan operations). Structure modifications to the index, which result in changing the size of revisions, happen through (lock-free) skip list node split and merge operations that are carefully coordinated with the update operations. Despite rich semantics, Jiffy offers highly scalable performance, which is comparable or exceeds the performance of the state-of-the-art lock-free ordered indices that feature linearizable range scan operations. Compared to its (lock-based) rivals that also support batch updates, Jiffy can execute large batch updates up to 7.4x more efficiently.

==> 2a-table-long.tex <==
\begin{table*}[t]
  \caption{Summary of properties of existing persistent data structures and
  LevelDB (as the reference implementation of a local data store).}
  \label{tab:systems}
  \begin{tabular}{l|clcc}
%     \toprule
     & Type & Concurrency scheme & Atomic batch writes & Atomic snapshots\\
    \midrule
    LevelDB \cite{LevelDB} & DRAM-HDD/SSD & multiple-reader, single-writer & \checkmark & \checkmark \\
    NoveLSM \cite{KBGA+18} & NVM-HDD/SSD & multiple-reader, single-writer & \checkmark & \checkmark \\
    SLM-DB \cite{KLNC19} & NVM-HDD/SSD & multiple-reader, single-writer & \checkmark & \\
    CDDS B-tree \cite{VTRC11} & NVM & multiple-reader, single-writer & \checkmark & possible, not implemented \\
    wB+Tree \cite{CJ15} & NVM & single-threaded & trivial & trivial \\
    BzTree \cite{ALML18} & NVM & PMwCAS & & \\
    FAST/FAIR \cite{DWYB18} & NVM & coarse-grained locks for writers (*) & & \\
    B3-tree \cite{CNJS+20} & NVM & coarse-grained locks for writers & & \\
    \texttt{csmap} \cite{PMDK} & NVM & fined-grained locks & &  \\
    NV-Tree \cite{YWCW+15}  & DRAM-NVM & coarse-grained locks for writers & & \\
    FPTree \cite{OLNW+16}  & DRAM-NVM & HTM + locks & & \checkmark \\ 
    HiKV \cite{XJXS17}  & DRAM-NVM & HTM + locks & &  \\
    FlatStore \cite{CLYW+20} & DRAM-NVM & & \\
    \kdb    & DRAM-NVM & coarse-grained locks for writers & \checkmark & \checkmark \\
    \bottomrule
        \multicolumn{5}{l}{* See details in \Cref{sec:related_work:all_nvm}.}\\
  \end{tabular}
\end{table*}

\endinput


==> 2a-table.tex <==
% \begin{minipage}{\textwidth}
% \scalebox{0.9}{
\begin{table*}[t]
  \caption{Summary of properties of selected persistent data stores (LevelDB as a baseline implementation).}
  \label{tab:systems}
%   \begin{tabular}{l|clp{1.6in}cc}
\begin{tabular}{l|cllcc}
%     \toprule
%      & & & & Atomic &  \\
     & Type & Architecture & Concurrency scheme & Batch updates & Snapshots\\
    \midrule
    \leveldb \cite{LevelDB} & DRAM-SS & SS-backed LSM Tree, skip list in DRAM & multiple-reader, single-writer & \checkmark & \checkmark \\
    \novelsm \cite{KBGA+18} & PM-SSD & PM-SSD LSM Tree & multiple-reader, single-writer & \checkmark & \checkmark \\
    \cdds \cite{VTRC11} & PM & B-tree & multiple-reader, single-writer & \checkmark & possible \\
    \texttt{csmap} \cite{PMDK} & PM & skip list & fined-grained locks & &  \\
    \nvtree \cite{YWCW+15}  & DRAM-PM & B+-tree, leafs in PM & coarse-grained locks for writers & & \\
    \fptree \cite{OLNW+16}  & DRAM-PM & B+-tree, leafs in PM & HTM + locks & & \checkmark$^{*}$ \\ 
    HiKV \cite{XJXS17}  & DRAM-PM & hash index in PM, asynchronously & HTM + locks & &  \\
    & & updated B+-tree in DRAM &  & &  \\
    FlatStore \cite{CLYW+20} & DRAM-PM & hash/Masstree index in DRAM, & keyset partitioned among CPU & \\
    & & log in PM & cores, user-level polling mech. & \\ 
    \utree \cite{CLFW+20} & DRAM-PM & B+-tree, leafs in PM & CAS in PM, locks in DRAM & &\\
    \kdb    & DRAM-PM & multi-skip-list in DRAM, entries in PM & coarse-grained locks for writers & \checkmark & \checkmark \\
    \bottomrule
    \multicolumn{6}{l}{* \fptree does not support snapshots (of the entire dataset), but its range scan operations are atomic.}\\
%         \multicolumn{5}{l}{* See details in \Cref{sec:related_work:all_nvm}.}\\
  \end{tabular}
\end{table*}
% }
% \end{minipage}

\endinput

\cite{VTRC11} \cite{YWCW+15} \cite{CJ15} \cite{OLNW+16} \cite{XJXS17} \cite{DWYB18} \cite{ALML18} \cite{KBGA+18} \cite{KLNC19} \cite{CNJS+20} \cite{CLYW+20}


\begin{table*}[t]
  \caption{Summary of properties of existing persistent data structures and
  LevelDB (as the reference implementation of a local data store).}
  \label{tab:systems}
  \begin{tabular}{l|clcc}
%     \toprule
     & Type & Concurrency scheme & Atomic batch writes & Atomic snapshots\\
    \midrule
    LevelDB \cite{LevelDB} & DRAM-HDD/SSD & multiple-reader, single-writer & \checkmark & \checkmark \\
%     NoveLSM \cite{KBGA+18} & PM-HDD/SSD & multiple-reader, single-writer & \checkmark & \checkmark \\
%     SLM-DB \cite{KLNC19} & PM-HDD/SSD & multiple-reader, single-writer & \checkmark & \\
%     CDDS B-tree \cite{VTRC11} & PM & multiple-reader, single-writer & \checkmark & possible, not implemented \\
%     wB+Tree \cite{CJ15} & PM & single-threaded & trivial & trivial \\
%     BzTree \cite{ALML18} & PM & PMwCAS & & \\
%     FAST/FAIR \cite{DWYB18} & PM & coarse-grained locks for writers (*) & & \\
%     B3-tree \cite{CNJS+20} & PM & coarse-grained locks for writers & & \\
    \texttt{csmap} \cite{PMDK} & PM & fined-grained locks & &  \\
    NV-Tree \cite{YWCW+15}  & DRAM-PM & coarse-grained locks for writers & & \\
    FPTree \cite{OLNW+16}  & DRAM-PM & HTM + locks & & \checkmark \\ 
    HiKV \cite{XJXS17}  & DRAM-PM & HTM + locks & &  \\
    FlatStore \cite{CLYW+20} & DRAM-PM & & \\
    \kdb    & DRAM-PM & coarse-grained locks for writers & \checkmark & \checkmark \\
    \bottomrule
%         \multicolumn{5}{l}{* See details in \Cref{sec:related_work:all_nvm}.}\\
  \end{tabular}
\end{table*}

\endinput


==> algorithms/apply_batch.tex <==
\begin{algorithm}[t] 
\caption{The $\applyBatch$ operation in \kdb}
\label{alg:applyBatch}  
% \algsetup{linenosize=\tiny}
%   \footnotesize
\small
% \vspace{-0.15cm}
% \begin{multicols*}{2}
\begin{algorithmic}[1]
\Procedure{$\applyBatch$}{$\batch$} 
   \State{\Var $\pDesc = \PersistentDescriptor(0)$} \label{alg:batchUpdate:pDesc} \LineComment{$\version = 0$}
   \State{$\pDesc.\persist()$} \label{alg:batchUpdate:pDescPersist}
   \State{\Var $\pEntryMap = \emptyset$}
   \For{$(\key,\val) \in \batch$} \label{alg:batchUpdate:persistLoop}
        \State{\Var $\pEntry = \PersistentBatchEntry(\key, \val, \pDesc)$} \label{alg:batchUpdate:pEntry}
        \State{$\pEntry.\persist()$}
        \State{$\pEntryMap.\pput(\key, \pEntry)$} 
   \EndFor \label{alg:batchUpdate:persistLoopEnd} 
   \State{\Var $\shardMap = \emptyset$}
   \For{$\key \in \batch.\keys()$} \label{alg:batchUpdate:batchLoop} \LineComment{ascending order} 
        \State{\Var $\shard = \findShard(\key)$}
        \State{$\shard.\lock()$} \LineComment{reentrant lock} 
        \State{$\shardMap.\pput(\key, \shard)$}
   \EndFor \label{alg:batchUpdate:batchLoopEnd}
   \State{\Var $\optVersion = -1 * \TSC.\rread()$} \label{alg:batchUpdate:optVersion}
   \State{$\pDesc.\version = \optVersion$} \label{alg:batchUpdate:pDescOptVersion}
   \State{$\pDesc.\persist()$} \label{alg:batchUpdate:pDescPersist2}
   \State{\Var $\vDesc = \VolatileDescriptor(0)$} \LineComment{$\version = 0$}
   \State{\Var $\vEntryList = \emptyset$}
   \For{$(\key,\pEntry) \in \pEntryMap$} \label{alg:batchUpdate:vEntryLoop}
       \State{\Var $\vEntry = \VolatileBatchEntry(\key, \pEntry, \optVersion, \vDesc)$}
       \State{$\shardMap.\get(\key).\add(\vEntry)$} \LineComment{as the first entry for key $\key$}
       \State{$\vEntryList.\append(\vEntry)$}
   \EndFor \label{alg:batchUpdate:vEntryLoopEnd}
   \State{$\vDesc.\version = \optVersion$}
   \State{\Var $\version = \TSC.\rread()$} \label{alg:batchUpdate:finalVersion}  \LineComment{guaranteed to be $> -\optVersion$}
   \State{$\vDesc.\casVersion(\optVersion, \version)$} \label{alg:batchUpdate:cas}
   \State{$\version = \vDesc.\version$}
   \State{$\pDesc.\version = \version$} \label{alg:batchUpdate:writeFinal}
   \State{$\pDesc.\persist()$} \label{alg:batchUpdate:flush2}
%    \State{wait until $\TSC.\rread() \ge \version$} \label{alg:batchUpdate:wait}
   \For{$\shard \in \shardMap.\values()$} \label{alg:batchUpdate:unlockLoop}
      \State{$\shard.\unlock()$} 
   \EndFor \label{alg:batchUpdate:unlockLoopEnd}
   \For{$\vEntry \in \vEntryList$} \label{alg:batchUpdate:versionCopyLoop} \LineComment{to speed-up future lookups and scans}
       \State{$\vEntry.\version = \version$}
   \EndFor \label{alg:batchUpdate:versionCopyLoopEnd} 
\EndProcedure
\end{algorithmic}
\end{algorithm}

\endinput




==> figures/skiplist_short.tex <==

% \newcommand{\shardColor}{lightgray}
% \newcommand{\dramColor}{blue}
% \newcommand{\pmColor}{red}

\definecolor{shardColor}{HTML}{2A2B2D}
\definecolor{dramColor}{HTML}{2DA8D8}
\definecolor{pmColor}{HTML}{D9514E}

\tikzstyle{arrow} = [->, thick, draw=dramColor]
\tikzstyle{parrow} = [->, thick, draw=pmColor]
\tikzstyle{small shard} = [rectangle, fill=dramColor]

\tikzstyle{shard style} = [ultra thick, draw=shardColor, fill=shardColor, fill opacity=0.03]
\tikzstyle{ventry shape} = [ultra thick, rectangle, draw=dramColor, fill=white, text=dramColor, minimum width=1cm, minimum height=0.5cm]
\tikzstyle{pentry shape} = [ultra thick, rectangle, draw=pmColor, fill=white, text=pmColor, minimum width=1cm, minimum height=0.5cm]
\tikzstyle{index shape} = [ultra thick, rectangle, draw=dramColor, fill=white, text=dramColor, minimum width=0.45cm, minimum height=0.45cm]
\tikzstyle{batch shape} = [ultra thick, circle, draw=pmColor, fill=white, text=pmColor, minimum size=0.4cm]

\newcommand{\smallShard}[2]{
   \node[label=above:#2] (#2) at ($ (#1) $) {};
%    \draw[|-|, very thick] ($ (#1) - (0.4, 0) $) -- ($ (#1) + (0.4, 0) $);
%    \draw[|-|, thick] ($ (#1) - (0.4, 0) $) -- ($ (#1) + (0.4, 0) $);
%    \fill [small shard] ($ (#1) - (0.4, 0.035) $) rectangle ($ (#1) + (0.4, 0.035) $);
}

\newcommand{\ventry}[3]{
   \node[ventry shape] (#1) at ($ (#2) $) {#3};
}

\newcommand{\pentry}[3]{
   \node[pentry shape] (#1) at ($ (#2) $) {#3};
}

\newcommand{\batch}[3]{
   \node[batch shape] (#1) at ($ (#2) $) {#3};
}


\newcommand{\idx}[3]{
   \node[index shape] (#1) at ($ (#2) $) {#3};
}

\bgroup
\begin{tikzpicture}[font=\sf\footnotesize] 

\newcommand{\ventryDist}{1.5}
\newcommand{\indexShift}{0.03}
\newcommand{\indexDist}{0.45}
\newcommand{\pentryVertDist}{1.2}
\newcommand{\batchVertDist}{2.1}

\node (startNode) at (0,0) {};

\node (c1) at ($(startNode) + (-\ventryDist/2, 5.2 * \indexDist)$) {};
\node (c2) at ($(startNode) + (8.5 * \ventryDist, 5.2 * \indexDist)$) {};
\node (c3) at ($(startNode) + (8.5 * \ventryDist, -2.2 * \pentryVertDist)$) {};
\node (c4) at ($(startNode) + (-\ventryDist/2, -2.2 * \pentryVertDist)$) {};

\draw[shard style] (c1.center) -- (c2.center) -- (c3.center) -- (c4.center) -- (c1.center);

\draw[ultra thick, dashed, draw=shardColor] ($ (startNode) + (-\ventryDist/2, -\pentryVertDist / 2)$) -- ($ (startNode) + (8.5 * \ventryDist, -\pentryVertDist / 2)$);

\node[text=dramColor] (label) at ($ (startNode) + (8 * \ventryDist, -0.3)$) {DRAM};
\node[text=pmColor] (label) at ($ (startNode) + (8 * \ventryDist, -0.9)$) {PM};

\node[text=dramColor] (label) at ($ (startNode) $) {vEntries:};
\ventry{e1}{$ (startNode) + (1 * \ventryDist, 0)$}{bla2}
\ventry{e2}{$ (startNode) + (2 * \ventryDist, 0)$}{bla2}
\ventry{e3}{$ (startNode) + (3 * \ventryDist, 0)$}{bla3}
\ventry{e4}{$ (startNode) + (4 * \ventryDist, 0)$}{bla4}
\ventry{e5}{$ (startNode) + (5 * \ventryDist, 0)$}{bla5}
\ventry{e6}{$ (startNode) + (6 * \ventryDist, 0)$}{bla6}
\ventry{e7}{$ (startNode) + (7 * \ventryDist, 0)$}{bla7}

\node[text=pmColor] (label) at ($ (startNode) + (0, -\pentryVertDist)$) {pEntries:};
\pentry{p1}{$ (startNode) + (1 * \ventryDist, -\pentryVertDist)$}{bla1}
\pentry{p2}{$ (startNode) + (2 * \ventryDist, -\pentryVertDist)$}{bla2}
\pentry{p3}{$ (startNode) + (3 * \ventryDist, -\pentryVertDist)$}{bla3}
\pentry{p4}{$ (startNode) + (4 * \ventryDist, -\pentryVertDist)$}{bla4}
\pentry{p5}{$ (startNode) + (5 * \ventryDist, -\pentryVertDist)$}{bla5}
\pentry{p6}{$ (startNode) + (6 * \ventryDist, -\pentryVertDist)$}{bla6}
\pentry{p7}{$ (startNode) + (7 * \ventryDist, -\pentryVertDist)$}{bla7}

\batch{b1}{$ (startNode) + (3 * \ventryDist, -\batchVertDist)$}{b}
\batch{b2}{$ (startNode) + (5.5 * \ventryDist, -\batchVertDist)$}{b}
\batch{b3}{$ (startNode) + (8 * \ventryDist, -\batchVertDist)$}{b}

\node (p8) at ($ (startNode) + (9 * \ventryDist, -\pentryVertDist)$) {};
\draw[parrow] (p2) -- (b1);
\draw[parrow] (p4) -- (b1);
\draw[parrow] (p5) -- (b2);
\draw[parrow] (p6) -- (b2);
\draw[parrow] (p7) -- (b3);
\draw[parrow, dashed] (p8) -- (b3);

\idx{i01}{$ (startNode) + (0.25 * \ventryDist, \indexShift + 1 * \indexDist)$}{}
\idx{i02}{$ (startNode) + (0.25 * \ventryDist, \indexShift + 2 * \indexDist)$}{}
\idx{i03}{$ (startNode) + (0.25 * \ventryDist, \indexShift + 3 * \indexDist)$}{}
\idx{i04}{$ (startNode) + (0.25 * \ventryDist, \indexShift + 4 * \indexDist)$}{H}

\idx{i11}{$ (startNode) + (1 * \ventryDist, \indexShift + 1 * \indexDist)$}{}
\idx{i12}{$ (startNode) + (1 * \ventryDist, \indexShift + 2 * \indexDist)$}{}
                                                                           
\idx{i21}{$ (startNode) + (2 * \ventryDist, \indexShift + 1 * \indexDist)$}{}
\idx{i22}{$ (startNode) + (2 * \ventryDist, \indexShift + 2 * \indexDist)$}{}
\idx{i23}{$ (startNode) + (2 * \ventryDist, \indexShift + 3 * \indexDist)$}{}
\idx{i24}{$ (startNode) + (2 * \ventryDist, \indexShift + 4 * \indexDist)$}{}
                                                                           
\idx{i31}{$ (startNode) + (3 * \ventryDist, \indexShift + 1 * \indexDist)$}{}
                                                                           
\idx{i41}{$ (startNode) + (4 * \ventryDist, \indexShift + 1 * \indexDist)$}{}
\idx{i42}{$ (startNode) + (4 * \ventryDist, \indexShift + 2 * \indexDist)$}{}
\idx{i43}{$ (startNode) + (4 * \ventryDist, \indexShift + 3 * \indexDist)$}{}
                                                                           
\idx{i51}{$ (startNode) + (5 * \ventryDist, \indexShift + 1 * \indexDist)$}{}
                                                                           
\idx{i61}{$ (startNode) + (6 * \ventryDist, \indexShift + 1 * \indexDist)$}{}
\idx{i62}{$ (startNode) + (6 * \ventryDist, \indexShift + 2 * \indexDist)$}{}
\idx{i63}{$ (startNode) + (6 * \ventryDist, \indexShift + 3 * \indexDist)$}{}
\idx{i64}{$ (startNode) + (6 * \ventryDist, \indexShift + 4 * \indexDist)$}{}
                                                                           
\idx{i71}{$ (startNode) + (7 * \ventryDist, \indexShift + 1 * \indexDist)$}{}
\idx{i72}{$ (startNode) + (7 * \ventryDist, \indexShift + 2 * \indexDist)$}{}
                                                                           
\idx{i81}{$ (startNode) + (7.75 * \ventryDist, \indexShift + 1 * \indexDist)$}{$\bot$}
\idx{i82}{$ (startNode) + (7.75 * \ventryDist, \indexShift + 2 * \indexDist)$}{$\bot$}
\idx{i83}{$ (startNode) + (7.75 * \ventryDist, \indexShift + 3 * \indexDist)$}{$\bot$}
\idx{i84}{$ (startNode) + (7.75 * \ventryDist, \indexShift + 4 * \indexDist)$}{$\bot$}

\draw[arrow] (i01) -- (i11);
\draw[arrow] (i11) -- (i21);
\draw[arrow] (i21) -- (i31);
\draw[arrow] (i31) -- (i41);
\draw[arrow] (i41) -- (i51);
\draw[arrow] (i51) -- (i61);
\draw[arrow] (i61) -- (i71);
\draw[arrow] (i71) -- (i81);

\draw[arrow] (i02) -- (i12);
\draw[arrow] (i12) -- (i22);
\draw[arrow] (i22) -- (i42);
\draw[arrow] (i42) -- (i62);
\draw[arrow] (i62) -- (i72);
\draw[arrow] (i72) -- (i82);

\draw[arrow] (i03) -- (i23);
\draw[arrow] (i23) -- (i43);
\draw[arrow] (i43) -- (i63);
\draw[arrow] (i63) -- (i83);

\draw[arrow] (i04) -- (i24);
\draw[arrow] (i24) -- (i64);
\draw[arrow] (i64) -- (i84);


\draw[parrow] (e1) -- (p1);
\draw[parrow] (e2) -- (p2);
\draw[parrow] (e3) -- (p3);
\draw[parrow] (e4) -- (p4);
\draw[parrow] (e5) -- (p5);
\draw[parrow] (e6) -- (p6);
\draw[parrow] (e7) -- (p7);



% \tikzstyle{dot} = [circle, fill, inner sep=1pt];
% 
% \newcommand{\dist}{0.9}
% 
% 
% \node (r1) at ($ (0, 1 * \procdist) + (-1.5, 0) $) [left] {$R_1$};
% \node (r2) at ($ (0, 0.5 * \procdist) + (-1.5, 0) $) [left] {$R_2$};
% \node (r3) at ($ (0, 0 * \procdist) + (-1.5, 0) $) [left] {$R_3$};
% \node (r4) at ($ (0, -0.5 * \procdist) + (-1.5, 0) $) [left] {$R_4$};
% 
% \draw [time line] (r1) -- (6.55 * \dist, 1 * \procdist);
% \draw [time line] (r2) -- (6.55 * \dist, 0.5 * \procdist);
% \draw [time line] (r3) -- (6.55 * \dist, 0.0 * \procdist);
% \draw [time line] (r4) -- (6.55 * \dist, -0.5 * \procdist);

\end{tikzpicture}
\egroup

